The LISE package: solvers for static and time-dependent superfluid local density approximation equations in three dimensions

Nuclear implementation of the density functional theory (DFT) is at present the only microscopic framework applicable to the whole nuclear landscape. The extension of DFT to superfluid systems in the spirit of the Kohn-Sham approach, the superfluid local density approximation (SLDA) and its extension to time-dependent situations, time-dependent superfluid local density approximation (TDSLDA), have been extensively used to describe various static and dynamical problems in nuclear physics, neutron star crust, and cold atom systems. In this paper, we present the codes that solve the static and time-dependent SLDA equations in three-dimensional coordinate space without any symmetry restriction. These codes are fully parallelized with the message passing interface (MPI) library and take advantage of graphic processing units (GPU) for accelerating execution. The dynamic codes have checkpoint/restart capabilities and for initial conditions one can use any generalized Slater determinant type of wave function. The code can describe a large number of physical problems: nuclear fission, collisions of heavy ions, the interaction of quantized vortices with nuclei in the nuclear star crust, excitation of superfluid fermion systems by time dependent external fields, quantum shock waves, domain wall generation and propagation, the dynamics of the Anderson-Bogoliubov-Higgs mode, dynamics of fragmented condensates, vortex rings dynamics, generation and dynamics of quantized vortices, their crossing and recombinations and the incipient phases of quantum turbulence.

==> code_running_test.tex <==
\section{Code Structure}

\subsection{Static Code}
%\texttt{get\_blcs\_dscr( MPI\_Comm gr\_comm, int m, int n, int mb, int nb, int p, int q, int * ip, int * iq, int *blcs\_dscr, int *miq, int *niq ) } : get the 2D block-cyclic distribution parameters.

%\begin{verbatim}
%make_ham()
%\end{verbatim}
%\texttt{get\_mem\_req\_blk\_cyc(int ip, int iq, int np, int nq, int ma, int na, int mblk, int nblk, int * nip, int * niq)}
\subsection{Time-dependent Code}

\section{Input and output}
\subsection{Static code}
In the static code, one needs to pass an input file to the executable. An example is the following \texttt{input.test.txt} file
\begin{verbatim}
nx 24
ny 24
nz 48
dx 1.25
dy 1.25
dz 1.25
broyden 0
coulomb 1
niter 1
N 146
Z 94
iext 0
force 1
pairing 1
alpha_mix 0.25
resc_dens 0
ecut 100.0
irun 0
print_wf 0
hbo 2.0
deform 0
q0 0.0
v0 0.0
z0 0.0
wneck 0.0
rneck 0.0
p 32
q 48
mb 40
nb 40
\end{verbatim}

\section{Utilities}

\section{Compilation and Running}




==> running_test.tex <==
\section{Code Structure}

\section{Input and output}

\section{Utilities}

\section{Compilation and Running}

\section{Test cases}


==> test_cases.tex <==
\section{Test cases} \label{sec:test}

The accuracy of the static code has been benchmarked in \cite{jin2017}

\subsection{Dynamical calculation: induced fission of $^{240}$Pu}
\begin{figure}[htbp]
\includegraphics[scale=0.5]{E_tot.pdf}
\end{figure}

==> utilities.tex <==
\section{Peformances}
